Isometric actions on locally compact finite rank median spaces

We prove that a connected locally compact median space of finite rank which admits a transitive action is isometric to $\mathbb{R}^n$ endowed with the $\ell^1$-metric. In the other side, replacing the transitivity assumption on the group of isometries by a certain regularity of the action on the compactification of the space, we show that all orbits are discrete. In our way to prove these results, we give a characterization of the compactness in complete median spaces of finite rank by the combinatorics of their halfspaces.

==> to_revisit <==
To do:
_Maybe add a picture for the example who shows that the join between closed subsets is not necessarely closed.
_Add in the introduction that the median spaces arise an asymptotic cones of mapping class group and hierarchically hyperbolic spaces. Cite Bowditch and Drutu-Sapir....
_Refers to the original article which shows the separation theorem.
_Give a more riguourous proof of Proposition 4.8.


_Define strongly separated in the last section.DONE
_Give a concrete definition of the set of halfspaces transverse to a subset.DONE
_Thick halfspaces. DONE
_Ask Indira about Haglund citation (2011 or 2021).DONE
_Metric completion of a locally compact median space is not necessarily locally compact, even if we assume the existance of a minimal action. Give an example in the case of reel tree.NOT NECESSARY
_One may simplify lemma 4.7 and the proof of the local compactness theorem by considering directly halfspaces lying in \HH_{x_0}. NOT REALLY
_Hopf-Rinow. DONE
_In duality subsection, add the property of the functors: sending product to co-coproduct. DONE
_Verify when the notion of join between convex subsets appeared and was connected to the convex hull in the finite rank case. DONE
_Poc set or poc set? DONE
_Make the subsection duality clearer. Give briefly definition and detail way concerning the ultrafilters and how they appear in the duality between median spaces and measured Poc set.DONE
_Change the notation from \Delta to \HH.DONE
_Add a remark regarding the fact that the convex hull of a compact subset in a locally convex median space with compact intervals is not necessarely compact.DONE
_Send back to Bowditch article for the notation of nthiterated join.DONE 

